Fairness Mediator: Neutralize Stereotype Associations to Mitigate Bias in Large Language Models

LLMs have demonstrated remarkable performance across diverse applications, yet they inadvertently absorb spurious correlations from training data, leading to stereotype associations between biased concepts and specific social groups. These associations perpetuate and even amplify harmful social biases, raising significant fairness concerns. To mitigate such biases, prior studies have attempted to project model embeddings into unbiased spaces during inference. However, these approaches have shown limited effectiveness due to their weak alignment with downstream social biases. Inspired by the observation that concept cognition in LLMs is primarily represented through a linear associative memory mechanism, where key-value mapping occurs in the MLP layers, we posited that biased concepts and social groups are similarly encoded as entity (key) and information (value) pairs, which can be manipulated to promote fairer associations. To this end, we propose Fairness Mediator (FairMed), a bias mitigation framework that neutralizes stereotype associations. Our framework comprises two main components: a stereotype association prober and an adversarial debiasing neutralizer. The prober captures stereotype associations encoded within MLP layer activations by employing prompts centered around biased concepts to detect the emission probabilities for social groups. Subsequently, the adversarial debiasing neutralizer intervenes in MLP activations during inference to equalize the association probabilities among different social groups. Extensive experiments across nine protected attributes show that FairMed significantly outperforms SOTA methods in effectiveness. Compared to the most effective baseline, FairMed presents competitive efficiency by cutting mitigation overhead by hundreds of minutes. FairMed also maintains the LLM's language understanding capabilities without compromising overall performance.

==> fig/1-intro.tex <==


\section{Introduction}

%liang2022holistic,
Large Language Models (LLMs) have rapidly advanced, achieving remarkable success across diverse natural language processing (NLP) tasks, such as question answering and text generation \cite{chiang2023vicuna,brown2020language,touvron2023llama2,radford2018improving}. These models are now deeply integrated into daily life, powering technologies like search engines \cite{xiong2024search} and virtual assistants \cite{dong2023towards}. Despite their successes, LLMs still face significant challenges related to robustness \cite{wang2021dual,liu2019perceptual,liu2020bias,tang2021robustart,liu2023towards}, privacy \cite{wang2023location,hu2023shield}, fairness \cite{xiao2024genderbias,li2024runner,wan2023biasasker}, and other trustworthiness concerns. This paper specifically focuses on the fairness issues associated with LLMs. LLMs often inherit social stereotypes and biases \cite{xiao2024genderbias} from the training data \cite{hofmann2024ai,sun2024fairness,wang2024new}, leading to biased behavior toward specific social groups, particularly in relation to protected attributes such as religion, race, and gender. For instance, GPT-3 \cite{brown2020language} has been shown to frequently associate Muslims with violent contexts \cite{abid2021persistent,inloes2024artificial}, and Microsoft's AI chatbot Tay infamously produced racist and inappropriate content after interacting with users on social media \cite{microsoft_chatbot}. As LLMs are increasingly integrated into socially sensitive software applications, developing effective bias mitigation techniques is critical to ensuring fairness and addressing growing concerns.


%,zhang2018mitigating,wang2021dynamically mitigate
Bias in LLMs often manifests as spurious correlations \cite{ramaswamy2021fair,geirhos2020shortcut,limisiewicz2023debiasing,hort2024bias} between \emph{biased concepts} (\eg, ``violence'') and specific \emph{social groups} (\eg, ``Muslim''), a phenomenon commonly referred to as stereotype associations \cite{hinton2017implicit,bijlstra2014stereotype}. These associations arise from the underrepresentation or skewed portrayal of certain social groups in training data, perpetuating harmful stereotypes and contributing to representational harm \cite{crawford2017trouble}, whereby systems reinforce the subordination of marginalized groups. Interestingly, such implicit associations and latent activation pathways have also been exploited in recent adversarial attacks \cite{kong2024patch, wang2025black, ying2024safebench}, backdoor attacks \cite{liang2023badclip, liang2024revisiting, liang2024vl}, jailbreak attacks \cite{ying2024jailbreak, ying2025reasoning, jing2025cogmorph} and hallucinations \cite{ho2024novo} against LLMs, revealing a broader category of vulnerabilities where malicious prompts or triggers activate specific undesired behaviors. To address these harmful stereotype associations (the root cause of biased behavior), numerous bias mitigation techniques have been proposed. While mitigation strategies applied during model training demand substantial computational resources \cite{lu2020gender,webster2020measuring}, several approaches \cite{ravfogel2020null,liang2020towards} have sought to improve efficiency by projecting model embeddings into unbiased subspaces during inference. However, these inference-time methods have shown limited effectiveness in mitigating downstream biased behaviors \cite{gallegos2024bias,delobelle2022measuring}, highlighting the need for a bias mitigation technique that can effectively address biases while maintaining computational efficiency in LLMs.


To address the limitation, we introduce Fairness Mediator (\toolns), a framework designed to effectively and efficiently mitigate stereotype associations during inference. Our approach is inspired by the linear associative memory mechanism within the multilayer perceptron (MLP) layers of LLMs \cite{meng2022locating,mengmass,kohonen1972correlation,anderson1972simple}, where inputs representing entities generate activations corresponding to the information linked to those entities \cite{meng2022locating}. We hypothesize that biased concepts and social groups are encoded similarly as entity (key) and information (value) pairs. By monitoring and intervening in this process, we aim to promote fairer associations. Our Fairness Mediator comprises two key components: a \emph{stereotype association prober}, which estimates the degree of bias in associations between concepts and social groups, and an \emph{adversarial debiasing neutralizer}, which adjusts the MLP activations to create neutral associations. The stereotype association prober begins by crafting templates focused on biased concepts to prompt the LLM to elicit responses from various social groups. By collecting the corresponding MLP activations as samples and the emitted probabilities of social groups as labels, we construct an auxiliary dataset. This dataset is then used to train simple fully connected networks to probe the stereotype associations, transforming complex activations into interpretable associations with social groups. To neutralize these associations, the adversarial debiasing neutralizer draws on techniques from adversarial attacks \cite{madry2017towards,goodfellow2014explaining}. By leveraging gradients from the prober, it iteratively adjusts the MLP activations to minimize disparities in association probabilities among social groups. These adjustments during inference decrease the likelihood of any social group being unfairly linked to biased concepts, thereby reducing the model’s reliance on harmful stereotypes and promoting fairer behavior.


% mediates
% v0
% To neutralize these stereotype associations, the adversarial debiasing neutralizer draws on techniques from adversarial attacks \cite{madry2017towards,goodfellow2014explaining}. It uses the gradients from the prober to iteratively modify the MLP activations, minimizing the disparity in association probabilities across social groups. Through adjustments during inference, our method reduces the likelihood of any social group being disproportionately linked to biased concepts, thus diminishing the model’s reliance on harmful stereotypes and leading to fairer behavior.

To evaluate the performance of our \toolns, we conduct extensive experiments across nine protected attributes using four popular chat LLMs from the renowned LLaMA family. Compared to six state-of-the-art bias mitigation methods, \tool demonstrates markedly superior effectiveness, achieving bias reductions of up to \revised{84.42\%} and 80.36\% in terms of $s_{\text{DIS}}$ and $s_{\text{AMB}}$, respectively, on average. Besides, \tool surpasses the most effective baseline (\ie, CDA \cite{lu2020gender}) in efficiency, cutting training time from 907.70 minutes to just 2.28 minutes while maintaining a slight advantage in inference speed, reducing it from 0.175 seconds to 0.152 seconds per bias-related query. Moreover, \tool preserves the LLM's language understanding capabilities without compromising overall performance, whereas CDA results in an average drop of 1.83\%. We conduct further investigations and empirically support our hypothesis that stereotype associations are encoded within specific MLP layer activations, primarily in the middle and deeper layers. Experiments on additional LLMs (\ie, BERT and BART) and other benchmarks (\ie, BiasAsker and Adult) further highlight the effectiveness and generalizability of our methods. Our main \textbf{contributions} are:



\begin{itemize} [leftmargin=2em]
% \vspace{-0.1in}
% \item We propose \textbf{Fairness Mediator}, an effective and efficient framework for debiasing LLMs by directly targeting stereotype associations within linear associative memory mechanisms.  

\item Building on the associative memory mechanism in MLP layers, we posit and empirically observe that stereotype associations are encoded similarly, leading us to propose \toolns, which identifies and intervenes in stereotype associations for effective bias mitigation.
\item We introduce a novel \emph{stereotype association prober} that captures bias encoded in MLP activations, and develop an \emph{adversarial debiasing neutralizer} that intervenes in activations during inference to achieve equal associations, thereby fostering fairer behavior in LLMs.
\item Extensive experiments demonstrate the effectiveness (average bias reductions of \revised{84.42\%} and 80.36\% for $s_{\text{DIS}}$ and $s_{\text{AMB}}$) and efficiency (hundreds of minutes saved compared to the most effective baseline) of our \toolns, all while preserving language understanding capabilities.
\item The codes and more results are publicly available on our website \cite{ourweb}.
\end{itemize}




% Extensive experiments across nine protected attributes demonstrate that our \tool significantly outperforms state-of-the-art methods in effectiveness, achieving average bias reductions of up to 84.42\% and 80.36\% for $s_{\text{DIS}}$ and $s_{\text{AMB}}$, respectively. Compared to the most effective baseline, \tool presents competitive efficiency by cutting mitigation overhead by hundreds of minutes. \tool also maintains the LLM's language understanding capabilities without compromising overall performance.


%generally falling into two categories: training-stage (\ie, adjusting model parameters during pre-training or fine-tuning)  and inference-stage approaches (\ie, manipulating model embeddings to project them into an unbiased subspace during inference) \cite{liang2020towards,ravfogel2020null}. However, the training-stage methods often demand substantial computational resources while the inference-stage approaches show limited effectiveness for downstream biased behaviors \cite{gallegos2024bias,delobelle2022measuring}, showing a critical need for a bias mitigation technique that effectively addresses bias while maintaining efficiency in LLMs.
 
 
 
 %. Training-stage methods mitigate bias by  while inference-stage methods \cite{liang2020towards,ravfogel2020null} mainly concentrate on manipulating model embeddings to project them into an unbiased subspace during inference. 

%, there is a critical need for a bias mitigation technique that effectively addresses bias while maintaining efficiency in LLMs.


%typically using techniques such as counterfactual data augmentation \cite{lu2020gender,barikeri2021redditbias}, regularization constraints \cite{webster2020measuring,park2023never}, or adversarial learning \cite{zhang2018mitigating,wang2021dynamically} to reduce biased associations. Although these approaches can be effective, they often demand substantial computational resources and involve lengthy training processes, limiting their practicality for large-scale models. Inference-stage methods \cite{liang2020towards,ravfogel2020null} mainly concentrate on manipulating model embeddings to project them into an unbiased subspace during inference, offering a more efficient and flexible approach to bias mitigation. However, the weak alignment of model embeddings with downstream biased behavior limits their overall effectiveness \cite{gallegos2024bias,delobelle2022measuring}, which is also shown in our evaluation results. Thus, there is a critical need for a bias mitigation technique that effectively addresses bias while maintaining efficiency in LLMs.


%To achieve the goal, our \tool consists of two components: a \emph{stereotype association prober} to estimate how biased concepts are associated with social groups, and an \emph{adversarial debiasing neutralizer} that intervenes in the MLP's activations to establish neutral associations.
%To derive the prober, we start by crafting templates centered around biased concepts to prompt the LLM to elicit social groups. We collect the corresponding activations as samples and the emitted probabilities of social groups as labels, constructing an auxiliary dataset, which is then used to train simple fully connected networks for each layer to probe the stereotype associations. The prober creates a link that transforms complex activations into social groups, offering direction for adjusting activations during inference. To neutralize stereotype associations, the adversarial debiasing neutralizer is designed inspired by adversarial attacks \cite{madry2017towards,goodfellow2014explaining}, leveraging the prober’s gradients to iteratively modify the MLP activations and minimize the disparity in association probabilities between social groups. By making subtle, controlled adjustments during inference, our approach prevents any group from being disproportionately linked to biased concepts while maintaining the model’s overall performance, leading to fairer outcomes. 


%Unlike traditional inference-stage methods that focus on model embeddings, our approach draws inspiration from the linear associative memory mechanism (key-value mapping) \cite{meng2022locating,mengmass,kohonen1972correlation,anderson1972simple} in the MLP layers of LLMs, where the MLP receives input activations representing entities and generates activations corresponding to the information associated with those entities. Therefore, to capture the stereotype associations encoded in LLMs, we could monitor the information flow within the MLP, treating biased concepts as keys and social groups as values. 
